Prompt Learning via Meta-Regularization

Pre-trained vision-language models have shown impressive success on various computer vision tasks with their zero-shot generalizability. Recently, prompt learning approaches have been explored to efficiently and effectively adapt the vision-language models to a variety of downstream tasks. However, most existing prompt learning methods suffer from task overfitting since the general knowledge of the pre-trained vision language models is forgotten while the prompts are finetuned on a small data set from a specific target task. To address this issue, we propose a Prompt Meta-Regularization (ProMetaR) to improve the generalizability of prompt learning for vision-language models. Specifically, ProMetaR meta-learns both the regularizer and the soft prompts to harness the task-specific knowledge from the downstream tasks and task-agnostic general knowledge from the vision-language models. Further, ProMetaR augments the task to generate multiple virtual tasks to alleviate the meta-overfitting. In addition, we provide the analysis to comprehend how ProMetaR improves the generalizability of prompt tuning in the perspective of the gradient alignment. Our extensive experiments demonstrate that our ProMetaR improves the generalizability of conventional prompt learning methods under base-to-base/base-to-new and domain generalization settings. The code of ProMetaR is available at https://github.com/mlvlab/ProMetaR.

==> Algorithms/pseudocode.tex <==
\begin{algorithm}
\caption{ProMetaR optimization algorithm}
\label{alg:psuedocode}
\begin{algorithmic}[1]
\State \textbf{Inputs:} $\boldsymbol{\Theta}, \boldsymbol{\phi}$, Dataset ${D}$
\State \textbf{Parameters:} $(\alpha, \beta, \gamma)$
\While{not converged}
    \State $\text{Sample a batch of datasets }{D}_k  \text{ from }D$
    
    \State $\boldsymbol{\Theta} \gets \boldsymbol{\Theta} - \gamma \nabla_{\boldsymbol{\Theta}} \left(\mathcal{L}\left(\boldsymbol{\Theta}; D_k\right) + \mathcal{R}\left(\boldsymbol{\Theta};D_k\right)\right)$
    \State $\left\{{D}^{\text{tr}}, {D}^{\text{val}}\right\} \gets {D}_k$
    % \For{$k = 1 \text{ to } K$}
        \State $\boldsymbol{g} \gets \nabla_{\boldsymbol{\Theta}} \mathcal{L}\left(\boldsymbol{\Theta}; {D}^{\text{tr}} \right)$
        % \State $g^{visclip} \gets \nabla_{\boldsymbol{\theta}^{vis}}\mathcal{L}^{clip}\left(\boldsymbol{\theta}^{vis}, \mathcal{D}^{(sup)}_k\right)$
        % \State $g^{txtreg} \gets \nabla_{\boldsymbol{\theta}^{txt}} \mathcal{L}^{txt}\left(\boldsymbol{\theta}^{txt}, \mathcal{D}^{(sup)}_k \right)$
        \State $\boldsymbol{g}_{\text{reg}} \gets \nabla_{\boldsymbol{\Theta}} \mathcal{R}\left(\boldsymbol{\Theta}; {D}^{\text{tr}} \right)$
        \State $\hat{\boldsymbol{\Theta}}\left(\phib \right) \gets \boldsymbol{\Theta} - \alpha \cdot \left(\boldsymbol{g}+\mathcal{M}^{\boldsymbol{\phi}}\left(\boldsymbol{g}_{\text{reg}};\boldsymbol{g}\right)\right)$
        % \State $\hat{\theta}^{txt}_k \gets \theta^{txt} - \alpha \cdot R^{\phi}\left(g^{txtclip}, g^{txtreg}\right)$
    % \EndFor

    % \State $g_k^{vis} \gets R^{\phi}\left(g^{visclip}, g^{visreg}\right)$
    % \State $g_k^{txt} \gets R^{\phi}\left(g^{txtclip}, g^{txtreg}\right)$
    \State ${\boldsymbol{\Theta}} \gets \boldsymbol{\Theta} -  \beta \cdot\nabla_{\boldsymbol{\Theta}}\mathcal{L}\left(\hat{\boldsymbol{\Theta}}\left(\phib \right); \text{Aug}\left({D}^{\text{val}}\right)\right)$
    \State $\boldsymbol{\phi} \gets \boldsymbol{\phi} - \beta \cdot \nabla_{\boldsymbol{\phi}}\mathcal{L}\left(\hat{\boldsymbol{\Theta}}\left(\boldsymbol{\phi} \right);\text{Aug}\left({D}^{\text{val}}\right)\right)$
    
    
\EndWhile
\State \textbf{return} $\boldsymbol{\Theta}, \boldsymbol{\phi}$
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}
% \caption{ProMetaR optimization algorithm (previous)}
% \begin{algorithmic}[1]
% \State \textbf{Inputs:} $\theta, \phi$, Datasets $\mathcal{D}$
% \State \textbf{Parameters:} learning rate $(\alpha, \beta, \gamma)$, inner iter $K$
% \For{$t=1 \text{ to } T$}
%     \State $\text{Sample a batch of datasets }\mathcal{D}_t  \text{ from }\mathcal{D}$
    
%     \State $\theta \gets \theta - \gamma \nabla_\theta \mathcal{L}\left(\theta, \mathcal{D}_t \right)$
%     \State $\left\{\mathcal{D}^{(sup)}_k, \mathcal{D}^{(qry)}_k\right\}_{k=1}^K \gets \mathcal{D}_t$
%     \For{$k = 1 \text{ to } K$}
%         \State $g_k \gets \nabla_{\boldsymbol{\theta}} \mathcal{L}\left(\boldsymbol{\theta}, \mathcal{D}^{(sup)}_k \right)$
%         \State $\hat{\theta}_k \gets \theta - \alpha \cdot g_k$
%     \EndFor

%     % \State $g_k^{vis} \gets R^{\phi}\left(g^{visclip}, g^{visreg}\right)$
%     % \State $g_k^{txt} \gets R^{\phi}\left(g^{txtclip}, g^{txtreg}\right)$
%     \State $\theta \gets \theta - \beta \cdot \sum_{k=1}^K \nabla_{\theta}\mathcal{L}^{clip}\left(\hat{\theta}_k, \text{Aug}\left(\mathcal{D}^{(qry)}_k\right)\right)$
%     % \State $\phi \gets \phi - \beta \cdot \sum_{k=1}^K \nabla_{\phi}\mathcal{L}^{clip}\left(\hat{\theta}_k, \text{Aug}\left(\mathcal{D}^{(qry)}_k\right)\right)$
    
    
% \EndFor
% \State \textbf{return} $\theta, \phi$
% \end{algorithmic}
% \end{algorithm}

==> Figures/tex/diagram_generalization.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=0.65\columnwidth]{Figures/image/generalization.pdf}
\caption{Traditional generalization and task generalization.
}
\label{fig:diagram}
\end{figure}

==> Figures/tex/fewshot.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=1.0\textwidth]{Figures/image/few-shot.pdf}
\caption{\textcolor{red}{Performance comparison on the few-shot learning settings with 8 datasets~($k=1,2,4,8,16$) (ing)}. 
}
\label{fig:fewshot}
\end{figure}

==> Tables/base2new-ori.tex <==
% main table 1 base to new generalization
% \usepackage{multirow}


\begin{table*}[ht]
  % \caption{\textbf{abbab.}
  % \centering
% \setlength{\tabcolsep}{6pt}
    % abcd
  % }
  \begin{subtable}{0.2\linewidth}
  \centering
  
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{69.34}   &   \textcolor{DarkGray}{74.22}   &   71.70 \\
    CoOp    &   \textcolor{DarkGray}{82.69}   &   \textcolor{DarkGray}{63.22}   &   71.66 \\
    CoCoOp  &   \textcolor{DarkGray}{80.47}   &   \textcolor{DarkGray}{71.69}   &   75.83 \\
    TKO    &   \textcolor{DarkGray}{81.13}    &   \textcolor{DarkGray}{75.00}    &   \textbf{77.78} \\
    
    \bottomrule
    \end{tabular}
    \caption{Average over 11 datasets}
    \label{tab:1.a}
  \end{subtable}
  \hfill
  \begin{subtable}{0.2\linewidth}
  \centering
  
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{72.43}   &   \textcolor{DarkGray}{68.14}   &   70.22 \\
    +CoOp    &   \textcolor{DarkGray}{76.47}   &   \textcolor{DarkGray}{67.88}   &   71.92 \\
    +CoCoOp  &   \textcolor{DarkGray}{75.98}   &   \textcolor{DarkGray}{70.43}   &   73.10 \\
    +RPO    &   \textcolor{DarkGray}{76.60}    &   \textcolor{DarkGray}{71.57}    &   \textbf{74.00} \\
    
    \bottomrule
  \end{tabular}
  \caption{ImageNet}
  \label{tab:1.b}
  \end{subtable}
  \hfill
  \begin{subtable}{0.2\linewidth}
  \centering
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{96.84}   &   \textcolor{DarkGray}{94.00}   &   95.40 \\
    \midrule
    +LP    &   \textcolor{DarkGray}{98.03}   &   \textcolor{DarkGray}{93.50}   &   95.71 \\
    +CoOp    &   \textcolor{DarkGray}{98.00}   &   \textcolor{DarkGray}{89.81}   &   93.73 \\
    +CoCoOp  &   \textcolor{DarkGray}{97.96}   &   \textcolor{DarkGray}{93.81}   &   95.84 \\
    +RPO     &   \textcolor{DarkGray}{97.97}  &   \textcolor{DarkGray}{94.37}    &   \textbf{96.03}  \\
    \bottomrule
  \end{tabular}
  \caption{Caltech101}
  \label{tab:1.c}
  \end{subtable}
  \hfill
  % \vspace{0.5em}
  \begin{subtable}{0.2\linewidth}
  \centering
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{91.17}   &   \textcolor{DarkGray}{97.26}   &   94.12 \\
    \midrule
    +LP    &   \textcolor{DarkGray}{94.87}   &   \textcolor{DarkGray}{92.50}   &   93.67 \\
    +CoOp    &   \textcolor{DarkGray}{93.67}   &   \textcolor{DarkGray}{95.29}   &   94.47 \\
    +CoCoOp  &   \textcolor{DarkGray}{95.20}   &   \textcolor{DarkGray}{97.69}   &   \textbf{96.43} \\
    +RPO    &   \textcolor{DarkGray}{94.63}   &   \textcolor{DarkGray}{97.50}    &   96.05  \\
    \bottomrule
  \end{tabular}
  \caption{OxfordPets}
  \label{tab:1.d}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{63.37}   &   \textcolor{DarkGray}{74.89}   &   68.65 \\
    \midrule
    +LP    &   \textcolor{DarkGray}{78.60}   &   \textcolor{DarkGray}{65.50}   &   71.45 \\
    +CoOp    &   \textcolor{DarkGray}{78.12}   &   \textcolor{DarkGray}{60.40}   &   68.13 \\
    +CoCoOp  &   \textcolor{DarkGray}{70.49}  &   \textcolor{DarkGray}{73.59}   &   72.01 \\
    +RPO    &   \textcolor{DarkGray}{73.87}   &  \textcolor{DarkGray}{75.53}    &  \textbf{74.69}\\
    \bottomrule
  \end{tabular}
  \caption{StanfordCars}
  \label{tab:1.e}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{72.08}   &   \textcolor{DarkGray}{77.08}   &   74.83 \\
    \midrule
    +LP    &   \textcolor{DarkGray}{97.87}   &   \textcolor{DarkGray}{65.87}   &   78.74 \\
    +CoOp    &   \textcolor{DarkGray}{97.60}   &  \textcolor{DarkGray}{59.67}   &   74.06 \\
    +CoCoOp  &   \textcolor{DarkGray}{94.87}   &   \textcolor{DarkGray}{71.75}   &   81.71 \\
    +RPO    &   \textcolor{DarkGray}{94.13}   &   \textcolor{DarkGray}{76.67}    &   \textbf{84.50}\\
    \bottomrule
  \end{tabular}
  \caption{Flowers102}
  \label{tab:1.f}
  \end{subtable}
  \hfill
  \vspace{0.5em}
  \begin{subtable}{0.3\linewidth}
  \centering
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{90.10}   &   \textcolor{DarkGray}{91.22}   &   90.66 \\
    \midrule
    +LP    &   \textcolor{DarkGray}{88.30}   &   \textcolor{DarkGray}{88.03}   &   88.17 \\
    +CoOp    &   \textcolor{DarkGray}{88.33}   &   \textcolor{DarkGray}{82.26}   &   85.19 \\
    +CoCoOp  &   \textcolor{DarkGray}{90.70}   &   \textcolor{DarkGray}{91.29}   &   \textbf{90.99} \\
   +RPO     &  \textcolor{DarkGray}{90.33}   &   \textcolor{DarkGray}{90.83}   &  90.58   \\
    \bottomrule
  \end{tabular}
  \caption{Food101}
  \label{tab:1.g}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{27.19}   &   \textcolor{DarkGray}{36.29}   &   31.09 \\
    \midrule
    +LP    &   \textcolor{DarkGray}{41.37}   &   \textcolor{DarkGray}{31.13}   &  35.53  \\
    +CoOp    &   \textcolor{DarkGray}{40.44}   &   \textcolor{DarkGray}{22.30}   &   28.75 \\
    +CoCoOp  &   \textcolor{DarkGray}{33.41}   &   \textcolor{DarkGray}{23.71}   &   27.74 \\
   +RPO     &   \textcolor{DarkGray}{37.33}  &    \textcolor{DarkGray}{34.20}   &  \textbf{35.70}   \\
    \bottomrule
  \end{tabular}
  \caption{FGVCAircraft}
  \label{tab:1.h}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{69.36}   &   \textcolor{DarkGray}{75.35}   &   72.23 \\
    \midrule
    +LP    &   \textcolor{DarkGray}{79.47}   &   \textcolor{DarkGray}{69.73}   &   74.28 \\
    +CoOp    &   \textcolor{DarkGray}{80.60}   &   \textcolor{DarkGray}{65.89}   &   72.51 \\
    +CoCoOp  &   \textcolor{DarkGray}{79.74}   &   \textcolor{DarkGray}{76.86}   &   78.27 \\
    +RPO    &    \textcolor{DarkGray}{80.60}   &  \textcolor{DarkGray}{77.80}     &  \textbf{79.18} \\
    \bottomrule
  \end{tabular}
  \caption{SUN397}
  \label{tab:1.i}
  \end{subtable}
  \hfill
  \vspace{0.5em}
  \begin{subtable}{0.3\linewidth}
  \centering
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{53.24}   &   \textcolor{DarkGray}{59.90}   &   56.37 \\
    \midrule
    +LP    &   \textcolor{DarkGray}{80.63}   &   \textcolor{DarkGray}{55.97}   &   66.07 \\
    +CoOp    &   \textcolor{DarkGray}{79.44}   &   \textcolor{DarkGray}{41.18}   &   54.24 \\
    +CoCoOp  &   \textcolor{DarkGray}{77.01}   &   \textcolor{DarkGray}{56.00}   &   64.85 \\
    +RPO     &   \textcolor{DarkGray}{76.70}    &   \textcolor{DarkGray}{62.13}    &  \textbf{68.61}  \\
    \bottomrule
  \end{tabular}
  \caption{DTD}
  \label{tab:1.j}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{56.48}   &   \textcolor{DarkGray}{64.05}   &   60.03 \\
    \midrule
    +LP    &   \textcolor{DarkGray}{82.30}   &   \textcolor{DarkGray}{68.00}   &  74.47  \\
    +CoOp    &   \textcolor{DarkGray}{92.19}   &   \textcolor{DarkGray}{54.74}   &   68.69 \\
    +CoCoOp  &   \textcolor{DarkGray}{87.49}   &   \textcolor{DarkGray}{60.04}   &   71.21 \\
    +RPO     &  \textcolor{DarkGray}{86.63}   &  \textcolor{DarkGray}{68.97}   &   \textbf{76.79}  \\
    \bottomrule
  \end{tabular}
  \caption{EuroSAT}
  \label{tab:1.k}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{70.53}   &  \textcolor{DarkGray}{77.50}   &   73.85 \\
    \midrule
    +LP    &   \textcolor{DarkGray}{85.27}   &   \textcolor{DarkGray}{73.53}   &  78.97  \\
    +CoOp    &   \textcolor{DarkGray}{84.69}   &   \textcolor{DarkGray}{56.05}   &   67.46 \\
    +CoCoOp  &   \textcolor{DarkGray}{82.33}   &   \textcolor{DarkGray}{73.45}   &   77.64 \\
    +RPO    &   \textcolor{DarkGray}{83.67}    &  \textcolor{DarkGray}{75.43}    &   \textbf{79.34}\\
    \bottomrule
  \end{tabular}
  \caption{UCF101}
  \label{tab:1.l}
  \end{subtable}
  \hfill
  \vspace{0.5em}
\caption{\textbf{Performance comparison on the base-to-new generalization setting.} We train our model with a subset of the classes (base classes) in a 16-shot setting and evaluate on the test set including base classes and new classes. H denotes the harmonic mean of base and novel performance to show the generalization trade-off~\cite{xian2017zero}.}
\label{tab:1}
\end{table*} 


==> Tables/base2new.tex <==
% main table 1 base to new generalization
\begin{table}[t]
  \centering
    \setlength{\tabcolsep}{2.5pt}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l c|c c c c c c c}
    % \begin{tabular}{ >{\arraybackslash}m{12mm}  >{\centering\arraybackslash}m{8mm} | >{\centering\arraybackslash}m{15mm}  >{\centering\arraybackslash}m{15mm}  >{\centering\arraybackslash}m{15mm}  >{\centering\arraybackslash}m{15mm}  >{\centering\arraybackslash}m{15mm}  >{\centering\arraybackslash}m{15mm}  >{\centering\arraybackslash}m{15mm} }
        \toprule
        \multirow{2}{*}{Dataset} & & CLIP & CoOp  & CoCoOp & MaPLe & PromptSRC & UNIGRAM & ProMetaR \\
        % \multirow{3}{*}{Dataset} & & \multirow{2}{*}{CLIP} & \multirow{2}{*}{CoOp}  & \multirow{2}{*}{CoCoOp} & \multirow{2}{*}{MaPLe} & \multirow{2}{*}{Prompt} & \multirow{2}{*}{UNI} & ProMetaR \\
         % & &  &  &  & & SRC & GRAM & ProMetaR \\
         & & \cite{radford2021learning} & \cite{zhou2022learning}  & \cite{zhou2022conditional} & \cite{khattak2023maple} &  \cite{khattak2023self} & \cite{li2023gradient} & (Ours) \\
        \midrule
        \midrule
        \multirow{4}{*}{\shortstack[l]{Average on\\11 datasets}} & Base & 69.34 & 82.69 & 80.47 & 82.28 & 84.26 & 80.34 & \\
         & New & 74.22 & 63.22 & 71.69 & 75.14 & 76.10 & 75.92 & \\
         & H & 71.70 & 71.66 & 75.83 & 78.55 & 79.97 & 78.07 & \\
         & Win & & & & & & & \\
         \midrule
         \multirow{3}{*}{ImageNet} & Base & 72.43 & 76.47 & 75.98 & 76.66 & 77.60 & 76.60 & \\
         & New & 68.14 & 67.88 & 70.43 & 70.54 & 70.73 & 70.69 & \\
         & H & 70.22 & 71.92 & 73.10 & 73.47 & 74.01 & 73.53 & \\
         \midrule
         \multirow{3}{*}{\shortstack[l]{Caltech\\101}} & Base & 96.84 & 98.00 & 97.96 & 97.74 & 98.10 & 98.07 & \\
         & New & 94.00 & 89.81 & 93.81 & 94.36 & 94.03 & 95.11 & \\
         & H & 95.40 & 93.73 & 95.84 &  96.02 & 96.02 & 96.57 & \\
         \midrule
         \multirow{3}{*}{\shortstack[l]{Oxford\\Pets}} & Base & 91.17 & 93.67 & 95.20 & 95.43 & 95.33 & 94.94 & \\
         & New & 97.26 & 95.29 & 97.69 & 97.76 & 97.30 & 97.94 & \\
         & H & 94.12 & 94.47 & 96.43 & 96.58 & 96.30 & 96.42 & \\
         \midrule
         \multirow{3}{*}{\shortstack[l]{Stanford\\Cars}} & Base & 63.37 & 78.12 & 70.49 & 72.94 & 78.27 & 73.50 & \\
         & New & 74.89 & 60.40 & 73.59 & 74.00 & 74.97 & 75.38 & \\
         & H & 68.65 & 68.13 & 72.01 & 73.47 & 76.58 & 74.43 & \\
         \midrule
         \multirow{3}{*}{\shortstack[l]{Flowers\\102}} & Base & 72.08 & 97.60 & 94.87 & 95.92 & 98.07 & 95.20 & \\
         & New & 77.80 & 59.67 & 71.75 & 72.46 & 76.50 & 76.21 & \\
         & H & 74.83 & 74.06 & 81.71 & 82.56 & 85.95 & 84.65 & \\
         \midrule
         \multirow{3}{*}{Food101} & Base & 90.10 & 88.33 & 90.70 & 90.71 & 90.67 & 90.84 & \\
         & New & 91.22 & 82.26 & 91.29 & 92.05 & 91.53 & 92.12 & \\
         & H & 90.66 & 85.19 & 90.99 & 91.38 & 91.10 & 91.48 & \\
         \midrule
         \multirow{3}{*}{\shortstack[l]{FGVC\\Aircraft}} & Base & 27.19 & 40.44 & 33.41 & 37.44 & 42.73 & 32.25 & \\
         & New & 36.29 & 22.30 & 23.71 & 35.61 & 37.87 & 38.00 & \\
         & H & 31.09 & 28.75 & 27.74 & 36.50 & 40.15 & 34.89 & \\
         \midrule
         \multirow{3}{*}{SUN397} & Base & 69.36 & 80.60 & 79.74 & 80.82 & 82.67 & 80.43 & \\
         & New & 75.35 & 65.89 & 76.86 & 78.70 & 78.57 & 77.91 & \\
         & H & 72.23 & 72.51 & 78.27 & 79.75 & 80.52 & 79.15 & \\
         \midrule
         \multirow{3}{*}{DTD} & Base & 53.24 & 79.44 & 77.01 & 80.36 & 83.37 & 73.62 & \\
         & New & 59.90 & 41.18 & 56.00 & 59.18 & 62.97 & 62.38 & \\
         & H & 56.37 & 54.24 & 64.85 & 68.16 & 71.75 & 67.56 & \\
         \midrule
         \multirow{3}{*}{EuroSAT} & Base & 56.48 & 92.19 & 87.49 & 94.07 & 92.90 & 86.26 & \\
         & New & 64.05 & 54.74 & 60.04 & 73.23 & 73.90 & 71.38 & \\
         & H & 60.03 & 68.69 & 71.21 & 82.35 & 82.32 & 78.12 & \\
         \midrule
         \multirow{3}{*}{UCF101} & Base & 70.53 & 84.69 & 82.33 & 83.00 & 87.10 & 82.00 & \\
         & New & 77.50 & 56.05 & 73.45 & 78.66 & 78.80 & 78.06 & \\
         & H & 73.85 & 67.46 & 77.64 & 80.77 & 82.74 & 79.98 & \\
    \bottomrule
    \end{tabular}
    }
  % \hfill
  % \vspace{0.5em}
\caption{\textbf{Performance comparison on the base-to-new generalization setting.} We train our model with a subset of the classes (base classes) in a 16-shot setting and evaluate on the test set including base classes and new classes. H denotes the harmonic mean of base and novel performance to show the generalization trade-off~\cite{xian2017zero}.}
\label{tab:1}
\end{table} 

==> Tables/base2novel_promptsrc.tex <==
\begin{table}[t!]
\centering
%
\tablestyle{-12pt}{1.1}
\addtolength{\tabcolsep}{+14pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lc|c c c c c c c}
\toprule
{Dataset} &  &  {CLIP} &  {CoOp} & {CoCoOp} &  {ProDA} & 
{MaPLe} & 
{PromptSRC} &  {$\Delta$}  \\
 & &  \cite{radford2021learning} & \cite{zhou2022learning} & \cite{zhou2022conditional}  & \cite{lu2022prompt}  & \cite{khattak2023maple}  & (Ours) & \\
\midrule
\multirow{3}{*}{\shortstack[l]{Average on\\  11 datasets}}       & Base      & 69.34  & 82.69   & 80.47  & 81.56   & 82.28        & \textbf{84.26}  &  \textcolor{MidnightBlue}{{+2.0}}\\
                               & Novel     & 74.22  & 63.22   & 71.69  & 72.30    & 75.14          & \textbf{76.10}  &   \textcolor{MidnightBlue}{{+1.0}}\\
                               & HM        & 71.70  & 71.66   & 75.83 &76.65     & 78.55        & \textbf{79.97}  &   \textcolor{MidnightBlue}{{+1.4}}\\
\midrule
\multirow{3}{*}{ImageNet}      & Base   & 72.43  & 76.47   &  75.98 &  75.40     & 76.66         & \textbf{77.60}  &  \textcolor{MidnightBlue}{{+0.9}}\\ 
                               & Novel    & 68.14  & 67.88   &  70.43 & 70.23      & 70.54       & \textbf{70.73}  &   \textcolor{MidnightBlue}{{+0.2}}\\ 
                               & HM          & 70.22  & 71.92   &  73.10 & 72.72   & 73.47     &\textbf{74.01}  &  \textcolor{MidnightBlue}{{+0.5}}\\
\midrule
\multirow{3}{*}{Caltech101}    & Base   & 96.84  & 98.00   &  97.96 & \textbf{98.27}   & 97.74          & 98.10 &   \textcolor{MidnightBlue}{{+0.4}}\\
                               & Novel     & 94.00  & 89.81   &  93.81 & 93.23   & \textbf{94.36}  & {94.03} & \textcolor{Bittersweet}{{-0.3}}\\
                               & HM          & 95.40  & 93.73   &  95.84 &  95.68  & \textbf{96.02} & \textbf{96.02} &  \textcolor{MidnightBlue}{{+0.0}}\\
\midrule
\multirow{3}{*}{OxfordPets}    & Base     & 91.17  & 93.67   & 95.20 & \textbf{95.43}       & \textbf{95.43 }      & {95.33}  &  \textcolor{Bittersweet}{{-0.1}}\\
                               & Novel      & 97.26  & 95.29   & {97.69} & \textbf{97.83}      & 97.76       & 97.30  &   \textcolor{Bittersweet}{{-0.5}}\\
                               & HM          & 94.12  & 94.47   & {96.43} & \textbf{96.62}      & 96.58        & 96.30  &   \textcolor{Bittersweet}{{-0.3}}\\
\midrule
\multirow{3}{*}{\shortstack[l]{Stanford \\ Cars}}  & Base    & 63.37 & 78.12    & 70.49 &74.70      & 72.94         & \textbf{78.27}  &  \textcolor{MidnightBlue}{{+5.3}}\\
                               & Novel     & 74.89 & 60.40    & 73.59& 71.20        & 74.00      & \textbf{74.97}  &  \textcolor{MidnightBlue}{{+1.0}}\\
                               & HM         & 68.65 & 68.13    & 72.01  &  72.91        & 73.47         & \textbf{76.58}  &  \textcolor{MidnightBlue}{{+3.1}}\\
\midrule
\multirow{3}{*}{Flowers102}    & Base     & 72.08 & 97.60    & 94.87  &97.70       & 95.92      &\textbf{98.07}  &  \textcolor{MidnightBlue}{{+2.1}}\\
                               & Novel     & \textbf{77.80} & 59.67    & 71.75 &68.68     & 72.46        & 76.50  & \textcolor{MidnightBlue}{{+4.1}}\\
                               & HM         & 74.83 & 74.06    & 81.71  & 80.66    & 82.56      & \textbf{85.95}  & \textcolor{MidnightBlue}{{+3.4}}\\
\midrule
\multirow{3}{*}{Food101}       & Base     & 90.10 & 88.33    & {90.70}  & 90.30    & \textbf{90.71 }      & 90.67  &\textcolor{Bittersweet}{{-0.1}}\\
                               & Novel     & 91.22 & 82.26    & 91.29  & 88.57       & \textbf{92.05}     &{91.53}  & \textcolor{Bittersweet}{{-0.5}}\\
                               & HM          & 90.66 & 85.19    & 90.99  & 89.43    & \textbf{91.38}   & {91.10}  & \textcolor{Bittersweet}{{-0.3}}\\
\midrule
\multirow{3}{*}{\shortstack[l]{FGVC \\ Aircraft}}  & Base    & 27.19 & 40.44    & 33.41 & 36.90    & 37.44       & \textbf{42.73}  &  \textcolor{MidnightBlue}{{+5.3}}\\
                               & Novel      & 36.29 & 22.30    & 23.71 &34.13      & 35.61      & \textbf{37.87}  &  \textcolor{MidnightBlue}{{+2.3}}\\
                               & HM         & 31.09 & 28.75    & 27.74  & 35.46    & 36.50   & \textbf{40.15}  &  \textcolor{MidnightBlue}{{+3.7}}\\
\midrule
\multirow{3}{*}{SUN397}        & Base    & 69.36 & 80.60    &  79.74  &78.67       & 80.82    &\textbf{82.67 } &   \textcolor{MidnightBlue}{{+1.9}}\\
                               & Novel      & 75.35 & 65.89    &  76.86 &76.93    & \textbf{78.70 }        & {78.47}  &  \textcolor{Bittersweet}{{-0.2}}\\
                               & HM        & 72.23 & 72.51    &  78.27 &77.79   & 79.75    & \textbf{80.52}  &  \textcolor{MidnightBlue}{{+0.8}}\\
\midrule
\multirow{3}{*}{DTD}           & Base    & 53.24 & 79.44    & 77.01 &80.67        & 80.36      & \textbf{83.37}  &  \textcolor{MidnightBlue}{{+3.0}}\\
                               & Novel     & 59.90 & 41.18    & 56.00 &56.48      & 59.18       & \textbf{62.97 } &  \textcolor{MidnightBlue}{{+3.8}}\\
                               & HM          & 56.37 & 54.24    & 64.85 &66.44    & 68.16      & \textbf{71.75}  & \textcolor{MidnightBlue}{{+3.6}}\\
\midrule
\multirow{3}{*}{EuroSAT}       & Base    & 56.48 & 92.19    & 87.49  &83.90        & \textbf{94.07}       & {92.90}  &  \textcolor{Bittersweet}{{-1.2}}\\
                               & Novel      & 64.05 & 54.74    & 60.04& 66.00      & 73.23      & \textbf{73.90}  & \textcolor{MidnightBlue}{{+0.7}}\\
                               & HM          & 60.03 & 68.69    & 71.21& 73.88  & \textbf{82.35}   & {82.32}  &  \textcolor{Bittersweet}{{-0.1}}\\
\midrule
\multirow{3}{*}{UCF101}        & Base     & 70.53  & 84.69   & 82.33  &85.23         & 83.00       &\textbf{ 87.10}  & \textcolor{MidnightBlue}{{+4.1}}\\
                               & Novel      & 77.50  & 56.05   & 73.45  &71.97     &78.66         & \textbf{78.80}  &  \textcolor{MidnightBlue}{{+0.1}}\\
                               & HM          & 73.85  & 67.46   & 77.64 &78.04   & 80.77    & \textbf{82.74}  & \textcolor{MidnightBlue}{{+2.0}}\\
\bottomrule
\end{tabular}%
}\vspace{-0.5em}
    \caption{\small\textnormal{Accuracy comparison on Base-to-novel generalization of PromptSRC with previous methods}. The prompts learned with our self-regularizing approach show overall consistent improvements on base classes, without losing generalization. Absolute gains over MaPLe \cite{khattak2023maple} are shown
    in \textcolor{MidnightBlue}{blue}.}
    \label{tab:base-to-new}
%\vspace{-5mm}
\end{table}

==> Tables/domain_generalization_ori.tex <==
% main table 2 - domain generalization

\begin{table*}[ht]
    \centering
    \caption{\textbf{Comparison of RPO, CoCoOp, CoOp and manual prompt in domain generalization.} RPO learns from ImageNet (16 images per class) and is evaluated by 4 datasets with distribution shift and ImageNet itself. RPO performs better on 4 out of 5 datasets compared to CoCoOp.}
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{} & & Source & \multicolumn{4}{c}{Target}  \\
          \cmidrule(r){3-3}\cmidrule(r){4-7}
          &{Learnable?} & {ImageNet} & {ImageNetV2} & {ImageNet-Sketch} & {ImageNet-A} & {ImageNet-R}\\
          \cmidrule(r){1-7}
        CLIP &  &  66.73 & 60.83 & 46.15 & 47.77 & 73.96\\
        +CoOp & \checkmark &  71.51 & 64.20 & 47.99 & 49.71 & 75.21\\
        +CoCoOp & \checkmark & 71.02 & 64.07 & 48.75 & \textbf{50.63} & 76.18\\
        \midrule
        +RPO & \checkmark &  \textbf{71.67} & \textbf{65.13} & \textbf{49.27} & \ 50.13 & \textbf{76.57} \\
        %\midrule
        %$\Delta$  & & +0.18 & +0.43 & +0.15 & %-0.73 & +0.42 \\
    \bottomrule
  \end{tabular}
  \label{tab:2}
\end{table*}

% Learnable 제외 Column -V2 -S -A -R Avg. 방식으로 전환해보기

==> Tables/reg_tab_manifold.tex <==
% \vspace{-7pt}
\begin{table}[ht]
  \centering
  \vspace{-10pt}
  \footnotesize
  % \renewcommand{\arraystretch}{0.9}
  \begin{tabular}{l|ccc}
    \toprule
    Method  & Base & New & H\\
    \midrule
    CoOp (+manifold mixup) & 80.55 & 70.45 & 75.16\\
    CoCoOp (+manifold mixup) & 80.29 & 72.54 & 76.22  \\
    Maple (+manifold mixup) & 82.93& 74.84& 78.68 \\
    PromptSRC (+manifold mixup) & 83.69& 75.90& 79.60 \\
    IVLP (base) (+manifold mixup) & 83.57 & 73.19 & 78.04  \\
    ProMetaR & \textbf{84.39}& \textbf{76.93}& \textbf{80.49} \\
    % PointNext & 87.7 & 87.0 & 70.5 \\
    \bottomrule
  \end{tabular}
\vspace{-10pt}
\caption{
\hjk{
Performance of prompting methods with manifold mixup. The results are average on 11 datasets.
}
}
\label{reb_tab:manifoldmix}
\vspace{-5pt}
\end{table} 


% \begin{table}[ht]
%   \centering
%   \small
%   \begin{tabular}{l|ccc}
%     \toprule
%     Method & SONN & ShapeNetPart & S3DIS\\
%     \midrule
%     \textbf{SPoTr} & \textbf{88.6} & \textbf{87.2} & \textbf{71.0}\\
%     w/o SPA & 87.9 & 86.9 & 69.9  \\
%     PointNet++ & 77.9& 85.1& 53.5 \\
%     % PointNext & 87.7 & 87.0 & 70.5 \\
%     \bottomrule
%   \end{tabular}
% \vspace{-7pt}
% \caption{Overall performance comparisons.}
% \label{reb_tab:manifoldmix}
% \vspace{-5pt}
% \end{table} 



==> notation.tex <==
\section*{Notation}

\begin{itemize}
    \item Textual embedding: $\Wb = \left\{\wb_c \right\}_{c=1}^{N_c}, \quad \wb_c = g(\pb_c)$
    \item Prompt augmented textual embedding : $\tilde{\Wb} = \left\{\tilde{\wb}_c \right\}_{c=1}^{N_c},\quad \tilde{\wb}_c = g(\tilde{\pb}_c)$
    \item Input of CLIP text encoder: $\pb_c = e(\texttt{"A photo of a [CLASS]"})$
    \item Image: $\mathbf{x}$
    \item Visual prompt: $\qb_i = \left[\eb_{\texttt{CLS}}, \eb_1, \dots, \eb_m \right]$
    \item Visual embedding: $\zb = f(\qb_i)$
    \item Visual prompt tuning: $\tilde{\zb} = f(\left[\eb_{\texttt{CLS}}, \ub_1, \dots, \ub_n, \eb_1, \dots, \eb_m \right])$
    \item Input of textencoder with prompt: $\tilde{\pb}_c = \left[\vb_1, \dots, \vb_m, \vb_{\texttt{CLASS}} \right]$
\end{itemize}
